Large Language Models for Stemming: Promises, Pitfalls and Failures

Text stemming is a natural language processing technique that is used to reduce words to their base form, also known as the root form. The use of stemming in IR has been shown to often improve the effectiveness of keyword-matching models such as BM25. However, traditional stemming methods, focusing solely on individual terms, overlook the richness of contextual information. Recognizing this gap, in this paper, we investigate the promising idea of using large language models (LLMs) to stem words by leveraging its capability of context understanding. With this respect, we identify three avenues, each characterised by different trade-offs in terms of computational cost, effectiveness and robustness : (1) use LLMs to stem the vocabulary for a collection, i.e., the set of unique words that appear in the collection (vocabulary stemming), (2) use LLMs to stem each document separately (contextual stemming), and (3) use LLMs to extract from each document entities that should not be stemmed, then use vocabulary stemming to stem the rest of the terms (entity-based contextual stemming). Through a series of empirical experiments, we compare the use of LLMs for stemming with that of traditional lexical stemmers such as Porter and Krovetz for English text. We find that while vocabulary stemming and contextual stemming fail to achieve higher effectiveness than traditional stemmers, entity-based contextual stemming can achieve a higher effectiveness than using Porter stemmer alone, under specific conditions.

==> gain_loss_analysis.tex <==
\subsection{Gain-loss analysis}

From Figure~\ref{fig:results.gain-loss}, it is evident that ECS.1 and Porter Stemmer perform similarly across a majority of queries with a few exceptions. One notable distinction lies in the processing of complex queries, where the performance margin tends to be more significant.

\textbf{Query 659}, which pertains to health and safety standards in cruise ships, when used porter stemmer, cruise is stemmed to cruis, however, cruise here is very important 


\subsection{Conclusion}
Our analysis reveals that while ECS.1 generally performs on par with the Porter Stemmer, its efficacy varies depending on the complexity and thematic elements of the queries. ECS.1-LlaMa-2 excels in scenarios where multiple themes are involved but struggles with queries requiring a nuanced understanding of specific domains. These findings suggest that while ECS.1-LlaMa-2 is promising, further research is needed to optimize its performance across a broader range of query types.




\begin{figure}[t!]
	\vspace{-12pt}
	\begin{subfigure}[t!]{.5\columnwidth}
		\includegraphics[width=\columnwidth]{plots/map_gain_loss_plot_1}
		\caption{ECS.1-LlaMa-2-Porter VS. Porter}
	\end{subfigure}
	\begin{subfigure}[t!]{.5\columnwidth}
		\includegraphics[width=\columnwidth]{plots/map_gain_loss_plot_2}
		\caption{ECS.2-LlaMa-2-Porter VS. Porter}
	\end{subfigure}
	\caption{Query by query gain-loss plot on Robust04-LAT, between ECS to Porter.}
	\label{fig:results.gain-loss}
	\vspace{-12pt}
\end{figure}

==> prompts_context.tex <==
\begin{tabular}{c|M{330pt}}
	\toprule
	Model & \textnormal{Prompt} \\
	\hline
	
%\rotatebox[origin=c]{90}{\parbox{1cm}{\centering ChatGPT}} &
%You are a professional in identifying entities given a paragraph. The entities can be names, brands, or organisations. 
%Can you extract all the entities from the following paragraph?\linebreak
%$\{sample\_paragraph\}$\linebreak
%Extracted entities:\linebreak
%$\{sample\_entities\_extracted\}$\linebreak
%Can you extract all the entities from the following paragraph?\linebreak
%$\{paragraph\}$ \linebreak Extracted entities:\\ \hline
%\linebreak \#\#\# Input: \hline

\rotatebox[origin=c]{90}{ChatGPT \& LlaMa-2-7b-chat} &You are a professional in identifying entities given a paragraph. The entities can be names, brands, or organisations. 
Can you extract all the entities from the following paragraph?\linebreak
$\{sample\_paragraph\}$\linebreak
Extracted entities:\linebreak
$\{sample\_entities\_extracted\}$\linebreak
Can you extract all the entities from the following paragraph?\linebreak
$\{paragraph\}$\linebreak Extracted entities:
\\
%	\rotatebox[origin=c]{90}{\parbox{1cm}{\centering ChatGPT}} &
%	You are a professional stemmer that is responsible to stem text. Text stemming is a natural language processing technique that is used to reduce words to their base form, also known as the root form. The process of stemming is used to normalize text and make it easier to process. You should stem every word except from names of people, places, organisations, brands. For example, the words `programming', `programmer', and `programs` can all be reduced down to the common stem `program'. However, in the sentence ``Programs PTY. LTD. sold for 1 billion euros'', the word `programs' should not be stemmed because it refers to the name of a company.\linebreak
%	Can you provide the stemmed version of this paragraph?\linebreak
%	$\{paragraph\_sample\}$\linebreak
%	Stemmed paragraph:\linebreak
%	$\{Stemmed\_paragraph\}$\linebreak
%	Can you provide the stemmed version of this paragraph?\linebreak
%	$\{paragraph\}$ \linebreak Stemmed paragraph:  \\ \hline
%	%\linebreak \#\#\# Input: \hline
%	
%	\rotatebox[origin=c]{90}{LlaMa-2-7b-chat} &You are a professional stemmer that is responsible to stem text. Text stemming is a natural language processing technique that is used to reduce words to their base form, also known as the root form. The process of stemming is used to normalize text and make it easier to process. You should stem every word except from names of people, places, organisations, brands. For example, the words `programming', `programmer', and `programs` can all be reduced down to the common stem `program'. However, in the sentence ``Programs PTY. LTD. sold for 1 billion euros'', the word `programs' should not be stemmed because it refers to the name of a company.\linebreak
%	Your output should strictly follow the format `original term:stemmed stems'. If a single original term produces multiple stems, separate produced stems with a space.\linebreak
%		Can you provide the stemmed version of this paragraph?\linebreak
%	$\{paragraph\_sample\}$\linebreak
%	Stemmed paragraph:\linebreak
%	$\{Stemmed\_paragraph\}$\linebreak
%	Can you provide the stemmed version of this paragraph?\linebreak
%	$\{paragraph\}$ \linebreak Stemmed paragraph:  
%	\\
	\bottomrule
\end{tabular}

==> related_work.tex <==
\section{Related Work}

\subsection{Traditional Stemming Techniques}
Stemming algorithms are foundational in the field of Information Retrieval (IR), and they are broadly classified into two main categories: \emph{algorithmic stemmers} and \emph{dictionary-based stemmers}.

\par{\textbf{Algorithmic stemmers}} like the Porter~\cite{porter1980algorithm} and Snowball~\cite{porter2001snowball} stemmers utilize rule-based heuristics to remove affixes from words. These methods are computationally efficient but often struggle with linguistic nuances and irregular word forms, leading to false positives. For example, the term $organisation$ is reduced to $organ$, which can be misleading.


\par{\textbf{Dictionary-based stemmers}} such as Krovetz~\cite{krovetz1993viewing} rely on a predefined list of word forms and their corresponding roots. These stemmers offer better linguistic accuracy but suffer from high rates of false negatives, particularly when encountering new or domain-specific terms.

\subsection{LLM in Information Retrieval}

In the IR filed, LLMs have been used for improving the effectiveness of ranking models. 
One group of methods involves harnessing the power of LLMs to augment training data, as demonstrated in studies such as~\cite{inpars,inparsv2,dai2023promptagator}. These approaches leverage LLMs to generate relevant queries, which are then used to train specialized ranking models.
Another line of research explores the direct prompting of LLMs for zero-shot document ranking, as exemplified by works like~\cite{gao2022precise,ma2023zero,pradeep2023rankvicuna,qin2023large,sachan-etal-2022-improving,sun2023chatgpt,zhuang2023setwise}. These techniques feed queries and documents as input to LLMs, employing various prompts to instruct the model to estimate relevance. Subsequently, the documents are ranked based on these estimations.
Furthermore, LLMs have been leveraged for relevance labeling~\cite{faggioli2023perspectives,thomas2023large}, showcasing remarkable alignment with human annotators. 
The work most closely aligned with this paper is doc2query~\cite{gospodinov2023doc2query,nogueira2019doc2query,nogueira2019document}. In these methodologies, LLMs are employed to generate relevant queries for each document, which are then appended into the original texts, thereby enhancing their content. Our approach also augments the original document text using LLMs, but in a zero-shot fashion. This stands in contrast to doc2query, which relies on a substantial volume of training data for its supervision. As a result, doc2query operates as a supervised method.


==> results-table-baseline.tex <==
\begin{tabular}{ll|llllll}
	\toprule
	Model & Setting&P& R &B-AC& F3 &Suc &WSS\\
	\hline \addlinespace[2pt]
\multirow{3}{*}{Bio-SIEVE} & Original/Calibrated& \textbf{0.232} & 0.576 & 0.727 & \textbf{0.429} & 0.111 & 0.858 \\\cmidrule{2-8} % \midrule
%\cmidrule{2-8}
 & Calibrated(Recall=0.95) & 0.102* & 0.877* & 0.683 & 0.348 & 0.481* & 0.471* \\ \cmidrule{2-8}
&Calibrated (Recall=1) & 0.088* & 0.945* & 0.666 & 0.339 & 0.704* & 0.369* \\ \midrule

\multirow{4}{*}{LlaMa-2-7b-inst}& Uncalibrated & 0.078* & 0.920* & 0.725 & 0.359 & 0.333 & 0.513* \\\cmidrule{2-8}
 & Calibrated (Recall=0.95) & 0.068* & 0.935* & 0.685 & 0.333 & 0.481* & 0.421* \\ \cmidrule{2-8}
 & Calibrated(Recall=1) & 0.059* & \textbf{0.990*} & 0.621* & 0.311 & \textbf{1.000}* & 0.241* \\ \midrule
%
%\multirow{4}{*}{LlaMa-2-13b-chat} &Uncalibrated  & 0.176 & 0.407* & 0.652* & 0.294* & 0.037 &0.886\\\cmidrule{2-8}
% & Cal (Recall=0.95) & 0.055* & 0.917* & 0.561* & 0.277* & 0.519* & 0.200* \\ \cmidrule{2-8}
% & Cal (Recall=1) & 0.051* & 0.973* & 0.528* & 0.278* & 0.741* & 0.080* \\ \midrule


\multirow{4}{*}{Ensemble} &Uncalibrated  & 0.400* & 0.204* & 0.594* & 0.199* & 0.037 & \textbf{0.972}* \\\cmidrule{2-8}
& Calibrated (Recall=0.95) & 0.095* & 0.937* & \textbf{0.729} & 0.373 & 0.519* & 0.500* \\ \cmidrule{2-8}
 & Calibrated (Recall=1) & 0.068* & 0.981* & 0.630* & 0.322 & 0.889* & 0.266* \\ \midrule
\end{tabular}

==> results-table-fusion.tex <==
\begin{tabular}{ll|llllllll}
	\toprule
	Dataset  & Model &Precision& Recall &B-AC&F0.5& F1& F3 &P(R90)&WSS\\
	\hline \addlinespace[2pt]
CLEF-2017 & fused & 0.077 & 0.920 & 0.726 & 0.093 & 0.134 & 0.353 & 0.055 & 0.516 \\
\midrule
CLEF-2018 & fused & 0.089 & 0.937 & 0.739 & 0.106 & 0.149 & 0.369 & 0.063 & 0.520 \\
\midrule
CLEF-2019-dta & fused & 0.104 & 0.881 & 0.727 & 0.118 & 0.153 & 0.329 & 0.027 & 0.552 \\
\midrule
CLEF-2019-intervention & fused & 0.082 & 0.918 & 0.699 & 0.097 & 0.137 & 0.344 & 0.049 & 0.463 \\
\midrule
Seed Collection & fused & 0.059 & 0.896 & 0.662 & 0.071 & 0.102 & 0.281 & 0.036 & 0.417 \\
\midrule
\end{tabular}


==> results-table-in-ex.tex <==
\begin{tabular}{ll|llllllll}
	\toprule
	
	Dataset& Model &Precision& Recall &B-AC&F0.5& F1& F3 &P(R90)& WSS \\
	\hline \addlinespace[2pt]
	clef-tar-CLEF-2017& llama-2-chat & 0.074 & 0.860 & 0.726 & 0.089 & 0.128 & 0.333 & 0.050 & 0.577 \\
	clef-tar-CLEF-2017& llama-2-chat & 0.061 & 0.910 & 0.666 & 0.074 & 0.108 & 0.306 & 0.042 & 0.411 \\\midrule
	clef-tar-CLEF-2017& llama-2-13b-chat & 0.185 & 0.397 & 0.660 & 0.184 & 0.201 & 0.292 & 0.005 & 0.912 \\
	clef-tar-CLEF-2017& llama-2-13b-chat & 0.241 & 0.338 & 0.647 & 0.224 & 0.225 & 0.284 & 0.000 & 0.944 \\\midrule
	
	clef-tar-CLEF-2018& llama-2-chat & 0.094 & 0.882 & 0.748 & 0.111 & 0.154 & 0.368 & 0.033 & 0.594 \\
	clef-tar-CLEF-2018& llama-2-chat & 0.102 & 0.880 & 0.711 & 0.118 & 0.158 & 0.356 & 0.052 & 0.521 \\\midrule
	clef-tar-CLEF-2018& llama-2-13b-chat & 0.257 & 0.364 & 0.659 & 0.245 & 0.249 & 0.303 & 0.000 & 0.940 \\
	clef-tar-CLEF-2018& llama-2-13b-chat & 0.333 & 0.362 & 0.666 & 0.285 & 0.273 & 0.321 & 0.019 & 0.958 \\\midrule
	
	clef-tar-CLEF-2019-dta& llama-2-chat & 0.092 & 0.922 & 0.714 & 0.109 & 0.149 & 0.346 & 0.072 & 0.492 \\
	clef-tar-CLEF-2019-dta& llama-2-chat & 0.088 & 0.924 & 0.676 & 0.103 & 0.142 & 0.340 & 0.073 & 0.416 \\\midrule
	clef-tar-CLEF-2019-dta& llama-2-13b-chat & 0.192 & 0.490 & 0.688 & 0.199 & 0.220 & 0.318 & 0.000 & 0.870 \\
	clef-tar-CLEF-2019-dta& llama-2-13b-chat & 0.226 & 0.427 & 0.661 & 0.224 & 0.233 & 0.301 & 0.000 & 0.880 \\\midrule
	
	clef-tar-CLEF-2019-intervention& llama-2-chat & 0.081 & 0.903 & 0.704 & 0.097 & 0.138 & 0.351 & 0.051 & 0.490 \\
	clef-tar-CLEF-2019-intervention& llama-2-chat & 0.087 & 0.875 & 0.692 & 0.103 & 0.145 & 0.358 & 0.031 & 0.493 \\\midrule
	clef-tar-CLEF-2019-intervention& llama-2-13b-chat & 0.181 & 0.476 & 0.682 & 0.186 & 0.213 & 0.343 & 0.005 & 0.873 \\
	clef-tar-CLEF-2019-intervention& llama-2-13b-chat & 0.263 & 0.524 & 0.716 & 0.256 & 0.281 & 0.397 & 0.019 & 0.888 \\\midrule
\end{tabular}


==> results-table-seed.tex <==
\begin{tabular}{ll|lllllll}
	\toprule
	
	Dataset& Model &Precision& Recall &B-AC&F0.5& F1& F3 &P(R90) \\
	\hline \addlinespace[2pt]
	%below for zero-shot
sysrev-seed-collection& llama & 0.036 & 0.871 & 0.467 & 0.044 & 0.066 & 0.209 & 0.029 \\
sysrev-seed-collection& llama-2 & 0.042 & 0.278 & 0.530 & 0.049 & 0.066 & 0.143 & 0.000 \\
sysrev-seed-collection& llama-2-13b & 0.037 & \textbf{0.975} & 0.489 & 0.045 & 0.068 & 0.222 & 0.037 \\
sysrev-seed-collection& falcon & 0.037 & 0.905 & 0.487 & 0.045 & 0.067 & 0.216 & 0.031 \\
sysrev-seed-collection& alpaca & 0.037 & 0.875 & 0.485 & 0.045 & 0.067 & 0.212 & 0.029 \\
sysrev-seed-collection& llama-2-chat & 0.052 & 0.881 & 0.646 & 0.063 & 0.092 & 0.268 & 0.036 \\
sysrev-seed-collection& llama-2-13b-chat & \textbf{0.124} & 0.467 & \textbf{0.666} & \textbf{0.128} & \textbf{0.150} & \textbf{0.272} & 0.002 \\
	\midrule
	%below for  average seed
sysrev-seed-collection& llama-seed & 0.035 & 0.868 & 0.467 & 0.043 & 0.065 & 0.207 & 0.027 \\
sysrev-seed-collection& llama-2-seed & 0.038 & 0.648 & 0.501 & 0.046 & 0.068 & 0.195 & 0.016 \\
sysrev-seed-collection& llama-2-13b-seed & 0.039 & 0.891 & 0.516 & 0.048 & 0.071 & 0.224 & 0.031 \\
sysrev-seed-collection& falcon-seed & 0.037 & 0.816 & 0.479 & 0.044 & 0.065 & 0.191 & 0.017 \\
sysrev-seed-collection& alpaca-seed & 0.021 & 0.316 & 0.269 & 0.026 & 0.036 & 0.096 & 0.007 \\
sysrev-seed-collection& llama-2-chat-seed & 0.039 & \textbf{0.893} & 0.514 & 0.048 & 0.072 & 0.226 & \textbf{0.031} \\
sysrev-seed-collection& llama-2-13b-chat-seed & \textbf{0.109} & 0.433 & \textbf{0.639} & \textbf{0.109} & \textbf{0.127} & \textbf{0.231} & 0.009 \\
	
	
	\midrule
	
%below for optimal seed for optimising B-AC
sysrev-seed-collection& llama-seed & 0.038 & 0.908 & 0.516 & 0.047 & 0.070 & 0.222 & 0.031 \\
sysrev-seed-collection& llama-2-seed & 0.047 & 0.744 & 0.589 & 0.057 & 0.083 & 0.231 & 0.026 \\
sysrev-seed-collection& llama-2-13b-seed & 0.044 & \textbf{0.914} & 0.577 & 0.054 & 0.079 & 0.243 & 0.030 \\
sysrev-seed-collection& falcon-seed & 0.040 & 0.854 & 0.512 & 0.048 & 0.069 & 0.201 & 0.020 \\
sysrev-seed-collection& alpaca-seed & 0.045 & 0.615 & 0.554 & 0.054 & 0.077 & 0.209 & 0.011 \\
sysrev-seed-collection& llama-2-chat-seed & 0.047 & 0.898 & 0.609 & 0.058 & 0.086 & 0.261 & \textbf{0.035} \\
sysrev-seed-collection& llama-2-13b-chat-seed & \textbf{0.145} & 0.651 & \textbf{0.748} & \textbf{0.156} & \textbf{0.194} & \textbf{0.374} & 0.014 \\
	
	\bottomrule
\end{tabular}

==> results-table-threshold-zero-shot.tex <==
\begin{minipage}[t]{0.45\textwidth}
	\centering
	\begin{adjustbox}{valign=t}
		
		\begin{tabular}{p{3pt}ll|llllll}
	\toprule
	& Model & Setting &P & R& B-AC&F3&Suc&WSS \\
	\hline \addlinespace[2pt]
\multirow{11}{*}{\rotatebox{90}{CLEF-2017}} & \multirow{3}{*}{\rotatebox{37}{7b-inst}} & Unc & 0.08 & 0.87 & 0.72 & 0.35 & 0.26 & 0.56\\
& & Cal(0.95) & 0.06* & 0.92* & 0.69* & 0.32 & 0.52 & 0.44 \\
& & Cal(1) & 0.05* & \textbf{0.99}* & 0.60* & 0.28 & 0.96 & 0.20 \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{13b-inst}} & Unc & 0.19 & 0.41 & 0.66 & 0.31 & 0.04 & 0.91\\
& & Cal(0.95) & 0.06* & 0.93 & 0.59* & 0.28 & 0.50* & 0.25* \\
& & Cal(1) & 0.05* & 0.98 & 0.53* & 0.26 & 0.88* & 0.08* \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{Ensemble}} & Unc & \textbf{0.31} & 0.13 & 0.56 & 0.13 & 0.00 & \textbf{0.98}\\
& & Cal(0.95) & 0.08 & 0.93* & \textbf{0.72} & \textbf{0.35}* & 0.52* & 0.50* \\
& & Cal(1) & 0.06 & 0.97* & 0.63 & 0.30 & \textbf{0.90}* & 0.29* \\
\midrule

\multirow{11}{*}{\rotatebox{90}{CLEF-2018}} & \multirow{3}{*}{\rotatebox{37}{7b-inst}} & Unc & 0.09 & 0.88 & 0.75 & 0.37 & 0.27 & 0.59\\
& & Cal(0.95) & 0.08* & 0.94* & 0.71* & 0.35* & 0.50 & 0.46 \\
& & Cal(1) & 0.06* & \textbf{0.99}* & 0.62* & 0.30 & \textbf{1.00} & 0.24 \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{13b-inst}} & Unc & 0.26 & 0.36 & 0.66 & 0.30 & 0.00 & 0.94\\
& & Cal(0.95) & 0.06 & 0.94* & 0.59* & 0.29 & 0.47* & 0.22* \\
& & Cal(1) & 0.05 & 0.97 & 0.53* & 0.27 & 0.80* & 0.08* \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{Ensemble}} & Unc & \textbf{0.35} & 0.12 & 0.54 & 0.12 & 0.00 & \textbf{0.95}\\
& & Cal(0.95) & 0.09* & 0.94* & \textbf{0.75} & \textbf{0.38}* & 0.50* & 0.54* \\
& & Cal(1) & 0.06 & 0.99* & 0.64 & 0.32* & 0.93* & 0.28* \\
\midrule

\multirow{11}{*}{\rotatebox{90}{CLEF-2019-dta}} & \multirow{3}{*}{\rotatebox{37}{7b-inst}} & Unc & 0.09 & 0.92 & 0.71 & \textbf{0.35} & 0.62 & 0.49\\
& & Cal(0.95) & 0.10* & 0.91* & 0.71* & 0.34 & 0.50 & 0.50 \\
& & Cal(1) & 0.08* & 0.97* & 0.66 & 0.32 & 0.75 & 0.34 \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{13b-inst}} & Unc & 0.19 & 0.49 & 0.69 & 0.32 & 0.00 & 0.87\\
& & Cal(0.95) & 0.08 & 0.95 & 0.56 & 0.29 & 0.50* & 0.16* \\
& & Cal(1) & 0.07 & 0.99 & 0.51 & 0.28 & 0.88* & 0.03* \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{Ensemble}} & Unc & \textbf{0.31} & 0.21 & 0.59 & 0.19 & 0.00 & \textbf{0.96}\\
& & Cal(0.95) & 0.10 & 0.91 & \textbf{0.73} & 0.34* & 0.50* & 0.52* \\
& & Cal(1) & 0.09* & \textbf{0.99} & 0.64 & 0.32* & \textbf{1.00}* & 0.28* \\
\midrule

\end{tabular}
\end{adjustbox}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
	\centering
\begin{adjustbox}{valign=t}
\begin{tabular}{lll|llllll}
	\toprule
& Model & Setting &P & R& B-AC&F3&Suc&WSS \\
\hline \addlinespace[2pt]
\multirow{11}{*}{\rotatebox{90}{CLEF-2019-Int}} & \multirow{3}{*}{\rotatebox{37}{7b-inst}} & Unc & 0.08 & 0.90 & 0.70 & 0.35 & 0.42 & 0.48\\
& & Cal(0.95) & 0.08* & 0.91* & 0.67* & 0.34 & 0.50 & 0.42 \\
& & Cal(1) & 0.07* & 0.93* & 0.64* & 0.33 & 0.65 & 0.34 \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{13b-inst}} & Unc & 0.17 & 0.45 & 0.67 & 0.33 & 0.05 & 0.87\\
& & Cal(0.95) & 0.07* & 0.90 & 0.58 & 0.30 & 0.50* & 0.25* \\
& & Cal(1) & 0.06* & 0.94 & 0.55 & 0.29 & 0.62* & 0.16* \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{Ensemble}} & Unc & \textbf{0.35} & 0.23 & 0.58 & 0.22 & 0.05 & \textbf{0.92}\\
& & Cal(0.95) & 0.09* & 0.93* & \textbf{0.70} & \textbf{0.37}* & 0.50* & 0.45* \\
& & Cal(1) & 0.08* &\textbf{0.96}* & 0.67 & 0.35* & \textbf{0.68}* & 0.35* \\

\midrule
\multirow{14}{*}{\rotatebox{90}{Seed Collection}} & \multirow{3}{*}{\rotatebox{37}{7b-inst}} & Unc & 0.05 & 0.90 & 0.66 & 0.27 & 0.54 & 0.40\\
& & Cal(0.95) & 0.05* & 0.90* & 0.66 & 0.28* & 0.51 & 0.41 \\
& & Cal(1) & 0.05* & 0.92* & 0.65 & 0.27* & 0.56 & 0.38 \\
 & & Cal (S) & 0.05 & 0.97* & 0.6* & 0.26 & 0.77* & 0.22* \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{13b-inst}} & Unc & 0.13 & 0.48 & 0.67 & 0.28 & 0.05 & 0.85\\
& & Cal(0.95) & 0.06* & 0.87 & 0.64* & 0.27* & 0.51* & 0.39* \\
& & Cal(1) & 0.05* & 0.93 & 0.59* & 0.26 & 0.59* & 0.25* \\
 & & Cal (S) & 0.06* & 0.87* & 0.63 & 0.29 & 0.54* & 0.38* \\
\cmidrule{2-9}
& \multirow{3}{*}{\rotatebox{37}{Ensemble}} & Unc & \textbf{0.16} & 0.18 & 0.52 & 0.14 & 0.00 & \textbf{0.86}\\
& & Cal(0.95) & 0.07* & 0.86* & \textbf{0.71} & 0.31* & 0.49* & 0.53* \\
& & Cal(1) & 0.07* & 0.88* & 0.70 & \textbf{0.30}* & 0.56* & 0.49* \\
& & Cal (S) & 0.04* & \textbf{1.00}* & 0.55 & 0.25* & \textbf{0.97}* & 0.10* \\
\midrule


\end{tabular}
\end{adjustbox}
\end{minipage}

==> results-table-zero-shot.tex <==
\begin{minipage}[t]{0.45\textwidth}
	\centering
\begin{adjustbox}{valign=t}
\begin{tabular}{p{3pt}l|llllll}
	\toprule
	& Model &P & R & B-AC&F3&Suc&WSS \\
	\hline \addlinespace[2pt]
\multirow{9}{*}{\rotatebox{90}{CLEF-2017}} & BioBERT & 0.06 & 0.95* & 0.61* & 0.30 & 0.74* & 0.26* \\\cmidrule{2-8}
& LlaMa-7b & 0.04* & 0.92* & 0.48* & 0.24* & 0.46* & 0.03* \\
& LlaMa-2-7b & 0.07 & 0.50* & 0.60* & 0.23* & 0.02* & 0.70* \\
& LlaMa-2-13b & 0.04* & 1.00* & 0.50* & 0.25* & 0.98* & 0.00* \\
& Falcon-7b-inst & 0.05* & 0.92* & 0.52* & 0.25* & 0.44 & 0.12* \\
& Alpaca-7b-inst & 0.04* & 0.92* & 0.51* & 0.25* & 0.38 & 0.11* \\
& LlaMa-2-7b-inst & 0.08 & 0.87 & \textbf{0.72} & \textbf{0.35} & 0.26 & 0.56 \\
& LlaMa-2-13b-inst & \textbf{0.19*} & 0.41* & 0.66* & 0.31 & 0.04* & \textbf{0.91*} \\
& Guanaco-7b-inst & 0.04* & \textbf{1.00*} & 0.50* & 0.25* & \textbf{1.00*} & 0.00* \\\midrule

\multirow{9}{*}{\rotatebox{90}{CLEF-2018}} & BioBERT & 0.06 & 0.97* & 0.59* & 0.29 & 0.87* & 0.19* \\\cmidrule{2-8}
& LlaMa-7b & 0.05* & 0.92* & 0.48* & 0.25* & 0.33 & 0.04* \\
& LlaMa-2-7b & 0.07 & 0.49* & 0.59* & 0.22* & 0.03* & 0.69* \\
& LlaMa-2-13b & 0.05* & 1.00* & 0.50* & 0.26 & \textbf{1.00*} & 0.00* \\
& Falcon-7b-inst & 0.05* & 0.92 & 0.51* & 0.25* & 0.40 & 0.11* \\
& Alpaca-7b-inst & 0.05* & 0.91 & 0.51* & 0.25* & 0.30 & 0.11* \\
& LlaMa-2-7b-inst & 0.09 & 0.88 & \textbf{0.75} & \textbf{0.37} & 0.27 & 0.59 \\
& LlaMa-2-13b-inst & \textbf{0.26*} & 0.36* & 0.66* & 0.30 & 0.00* & \textbf{0.94*} \\
& Guanaco-7b-inst & 0.05* & \textbf{1.00*} & 0.50* & 0.26 & \textbf{1.00*} & 0.00* \\\midrule
\multirow{9}{*}{\rotatebox{90}{CLEF-2019-dta}} & BioBERT & 0.07 & 0.99 & 0.58 & 0.30 & 0.88 & 0.18* \\\cmidrule{2-8}
& LlaMa-7b & 0.07 & 0.93 & 0.48* & 0.27 & 0.25 & 0.03* \\
& LlaMa-2-7b & 0.08 & 0.48* & 0.58* & 0.23 & 0.00* & 0.68 \\
& LlaMa-2-13b & 0.07 & 1.00 & 0.50* & 0.28 & \textbf{1.00} & 0.00* \\
& Falcon-7b-inst & 0.07 & 0.95 & 0.54* & 0.29 & 0.50 & 0.12* \\
& Alpaca-7b-inst & 0.07 & 0.91 & 0.52* & 0.28 & 0.25 & 0.12* \\
& LlaMa-2-7b-inst & 0.09 & 0.92 & \textbf{0.71} & \textbf{0.35} & 0.62 & 0.49 \\
& LlaMa-2-13b-inst & \textbf{0.19} & 0.49* & 0.69 & 0.32 & 0.00* & \textbf{0.87*} \\
& Guanaco-7b-inst & 0.07 & \textbf{1.00} & 0.50* & 0.28 & \textbf{1.00} & 0.00* \\\midrule
\end{tabular}
\end{adjustbox}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
	\centering
\begin{adjustbox}{valign=t}
\begin{tabular}{p{3pt}l|llllll}
	\toprule
	& Model &P & R& B-AC&F3&Suc&WSS \\
	\hline \addlinespace[2pt]
	\multirow{9}{*}{\rotatebox{90}{CLEF-2019-Int}} & BioBERT & 0.10 & 0.98* & 0.58* & 0.32 & 0.90* & 0.16* \\\cmidrule{2-8}
	& LlaMa-7b & 0.05* & 0.86 & 0.47* & 0.26 & 0.30 & 0.08* \\
	& LlaMa-2-7b & 0.08 & 0.30* & 0.55* & 0.18* & 0.05* & 0.80* \\
	& LlaMa-2-13b & 0.05 & 1.00* & 0.50* & 0.29 & 0.97* & 0.00* \\
	& Falcon-7b-inst & 0.05 & 0.91 & 0.50* & 0.27 & 0.57 & 0.09* \\
	& Alpaca-7b-inst & 0.05 & 0.87 & 0.49* & 0.27 & 0.30 & 0.12* \\
	& LlaMa-2-7b-inst & 0.08 & 0.90 & \textbf{0.70} & \textbf{0.35} & 0.42 & 0.48 \\
	& LlaMa-2-13b-inst & \textbf{0.17*} & 0.45* & 0.67 & 0.33 & 0.05* & \textbf{0.87*} \\
	& Guanaco-7b-inst & 0.05 & \textbf{1.00*} & 0.50* & 0.29 & \textbf{1.00*} & 0.00* \\\midrule
	\multirow{9}{*}{\rotatebox{90}{Seed Collection}} & BioBERT & 0.04 & 0.93 & 0.54* & 0.24 & 0.77* & 0.16* \\\cmidrule{2-8}
	& LlaMa-7b & 0.04 & 0.89 & 0.48* & 0.21 & 0.56 & 0.07* \\
	& LlaMa-2-7b & 0.04 & 0.29* & 0.53* & 0.15* & 0.03* & 0.78* \\
	& LlaMa-2-13b & 0.04 & \textbf{1.00*} & 0.50* & 0.23 & \textbf{1.00*} & 0.00* \\
	& Falcon-7b-inst & 0.04 & 0.93 & 0.50* & 0.22 & 0.69 & 0.07* \\
	& Alpaca-7b-inst & 0.04 & 0.90 & 0.50* & 0.22 & 0.49 & 0.10* \\
	& LlaMa-2-7b-inst & 0.05 & 0.90 & 0.66 & 0.27 & 0.54 & 0.40 \\
	& LlaMa-2-13b-inst & \textbf{0.13*} & 0.48* & \textbf{0.67} & \textbf{0.28} & 0.05* & \textbf{0.85*} \\
	& Guanaco-7b-inst & 0.04 & \textbf{1.00*} & 0.50* & 0.23 & \textbf{1.00*} & 0.00* \\\midrule
\end{tabular}
\end{adjustbox}
\end{minipage}


==> table_prompts.tex <==
\begin{tabular}{c|M{330pt}}
\toprule
Model & \textnormal{Prompt} \\
\hline
\rotatebox[origin=c]{90}{Alpaca} & Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \linebreak \#\#\# Instruction:\linebreak 
Answer `yes' or `no'\ to Judge if the following retrieved study should be included by the systematic review? 
\linebreak \#\#\# Input: 
\linebreak Review: ${review\_title}$\linebreak Study: ${candidate\_document}$ \linebreak
\#\#\# Response: \\\hline

\rotatebox[origin=c]{90}{\parbox{1cm}{\centering All Other Models}} & %Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \linebreak \#\#\# Instruction:\linebreak 
Answer `yes' or `no'\ to Judge if the following retrieved study should be included by the systematic review? 
%\linebreak \#\#\# Input: 
\linebreak Review: ${review\_title}$\linebreak Study: ${candidate\_document}$ \linebreak
%\#\#\# Response:
The answer is $`$\\
\bottomrule


%\rotatebox[origin=c]{90}{Title+\allowbreak Inc/\allowbreak Exc}&
%%Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \linebreak \#\#\# Instruction:\linebreak 
%Answer `yes' or `no'\ to Judge if the following retrieved study should be included by the systematic review, provided the review topic, inclusion and exclusion criteria? 
%%\linebreak \#\#\# Input:
%\linebreak Review: ${review\_title}$\linebreak Inclusion criteria: ${inclusion\_criteria}$
%\linebreak Exclusion criteria: ${exclusion\_criteria}$ \linebreak
%The answer is $`$
%%\#\#\# Response: 
%\\\hline
%\rotatebox[origin=c]{90}{Title+\allowbreak Seed} & 
%%Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \linebreak \#\#\# Instruction:\linebreak 
%Answer `yes' or `no'\ to Judge if the following retrieved study should be included by the systematic review, provided the review topic, inclusion and exclusion criteria?
%% \linebreak \#\#\# Input: 
%\linebreak Review: ${review\_title}$\linebreak Seed Study: ${seed\_study}$ \linebreak Retrieved Study: ${candidate\_document}$ \linebreak
%%\#\#\# Response:
%The answer is $`$ \\
\end{tabular}
%%% NOTE: Old version.
%	\begin{tabular}{p{25pt}|p{70pt}|M{300pt}}
%	Model   & Input Type & Prompt \\
%	\hline
%	\multirow{30}{*}{Alpaca} & Title Only & Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \linebreak \#\#\# Instruction:\linebreak Answer `yes' or `no'\ to Judge if the following retrieved study should be included by the systematic review? \linebreak \#\#\# Input: \linebreak Review: ${review\_title}$\linebreak Study: ${candidate\_document}$ \linebreak\#\#\# Response:
%	\\\cmidrule{2-3}
%	& Title+\allowbreak Inclusion/Exclusion&Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \linebreak \#\#\# Instruction:\linebreak Answer `yes' or `no'\ to Judge if the following retrieved study should be included by the systematic review, provided the review topic, inclusion and exclusion criteria? \linebreak \#\#\# Input: \linebreak Review: ${review\_title}$\linebreak Inclusion criteria: ${inclusion\_criteria}$\linebreak Exclusion criteria: ${exclusion\_criteria}$ \linebreak\#\#\# Response: \\\cmidrule{2-3}
%	& Title+\allowbreak seed study & Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \linebreak \#\#\# Instruction:\linebreak Answer `yes' or `no'\ to Judge if the following retrieved study should be included by the systematic review, provided the review topic, inclusion and exclusion criteria? \linebreak \#\#\# Input: \linebreak Review: ${review\_title}$\linebreak Seed Study: ${seed\_study}$ \linebreak Retrieved Study: ${candidate\_document}$ \linebreak\#\#\# Response:  \\
%	\hline
%	\multirow{20}{*}{Other} & Title Only & Answer the following 'yes' or 'no' question, should the following retrieved study being included in the systematic review?\linebreak Review: ${review\_title}$\linebreak Study: ${candidate\_document}$ \linebreak The answer is $`$
%	\\\cmidrule{2-3}
%	& Title+\allowbreak Inclusion/Exclusion & Answer the following 'yes' or 'no' question, should the following retrieved study being included in the systematic review, provided the review topic, inclusion and exclusion criteria?\linebreak Review: ${review\_title}$\linebreak Inclusion criteria: ${inclusion\_criteria}$\linebreak Exclusion criteria: ${exclusion\_criteria}$\linebreak Study: ${candidate\_document}$ \linebreak The answer is $`$
%	\\\cmidrule{2-3}
%	& Title+\allowbreak seed study  & Answer the following 'yes' or 'no' question, should the following retrieved study being included in the systematic review, provided the review topic, and one seed study of the review?\linebreak Review: ${review\_title}$\linebreak Seed Study: ${seed\_study}$\linebreak Retrieved Study: ${candidate\_document}$ \linebreak The answer is $`$ \\
%	% ... Repeat for other models
%\end{tabular}
